Learning to Ask Screening Questions for Job Postings

At LinkedIn, we want to create economic opportunity for everyone in the global workforce. A critical aspect of this goal is matching jobs with qualified applicants. To improve hiring efficiency and reduce the need to manually screening each applicant, we develop a new product where recruiters can ask screening questions online so that they can filter qualified candidates easily. To add screening questions to all $20$M active jobs at LinkedIn, we propose a new task that aims to automatically generate screening questions for a given job posting. To solve the task of generating screening questions, we develop a two-stage deep learning model called Job2Questions, where we apply a deep learning model to detect intent from the text description, and then rank the detected intents by their importance based on other contextual features. Since this is a new product with no historical data, we employ deep transfer learning to train complex models with limited training data. We launched the screening question product and our AI models to LinkedIn users and observed significant impact in the job marketplace. During our online A/B test, we observed $+53.10\%$ screening question suggestion acceptance rate, $+22.17\%$ job coverage, $+190\%$ recruiter-applicant interaction, and $+11$ Net Promoter Score. In sum, the deployed Job2Questions model helps recruiters to find qualified applicants and job seekers to find jobs they are qualified for.

==> bodyBackup.tex <==
\section{Introduction}

One of the core services at LinkedIn is to let recruiters post jobs on the job posting platform and also allow job applicants to apply for posted jobs. The general workflow of this is that the recruiters post jobs on job posting platform at LinkedIn with the job description, job requirements etc.; then whoever is interested in the job apply for it; and finally job posters should nail down the qualified candidate pool by choosing people whose profile and background meets the job requirements.

A common pain point for recruiters in the process is that they have to invest time in manually evaluating the applicants one by one to decide who are unqualified due to not meeting basic qualifications for a role. In most of the time, the review process is tedious and time consuming because the job applicants’ profile may be incomplete, out-dated, or just contains too much information for recruiters to read. It is also estimated that 70\% of phone screens end up with the recruiter finding out the candidate isn't eligible for the job due to obvious reasons such as lack of work authorization/visa. Therefore, it would significantly improves the hiring efficiency if job posting platforms such as LinkedIn can provide a way to simplify the applicant assessment process and let recruiters filter or sort applicants based on the assessment result easily.

To simplify the applicant assessment process, we decided to add a virtual screening session into the online application process. When job applicants apply for a job on LinkedIn, they need to answer a list of screening questions provided by the job posters. With these answers, the job posters or our AI models will be able to assess the applicants accordingly. 

Compared to other job applicant assessment methods such as analyzing their ability and experience level based on their LinkedIn profile or resume, this novel, question-based online screening process can precisely assess the job applicants based on job-specific questions and collect up-to-date answers from applicants directly. To help job posters better categorize the applicants based on different types of screening questions, each screening question should have a clear intent (e.g., work authorization, degree, skill experience) and a unified representation to avoid ambiguity across different jobs. Therefore we use structured screening questions in the format of (template, parameter) pairs instead of free from text. For example, all education degree questions about bachelor’s degree will be in the same format of (Have you completed the following level of education, Bachelor’s Degree).

After letting job posters manually add screening questions to jobs, we found that jobs with screening questions have significantly higher interaction rates. Based on most recent performance evaluations, jobs with screening questions yield 1.9x interactions (mutual interest between poster and applicant) overall, and 2.4x interactions with pre-screening qualified applicants. The increased interactions indicate that these screening questions bridge the communication between recruiters and applicants which enables great hiring efficiency.

Besides helping recruiters finding qualified applicants, the screening questions and the applicant provided answers can also be used to power job recommender systems and help us better understand the qualifications for job postings. For example, when a job applicant does not qualify for a specific job, we can recommend other similar jobs that she may qualify by matching the screening questions and her answers. By collecting and analyzing the correlations between recruiters’ actions and job applicants’ answers to the screening questions, we can better understand what qualifications are crucial to a specific role and what are optional.

However, the rate of jobs and applicants that were benefit from the screening questions are low --  the screening is only enabled for jobs that are created on LinkedIn, which constitute 4\% of total jobs, collecting more than 30\% of all applications. When a member applies to a pre-screening enabled job, LinkedIn prompts to save the answers, where 93\% of members opt in. This results in low coverage of the jobs that has screening questions enabled but high coverage of answers from job applicants for jobs that has screening questions. These observations create the motivation for building a system that can infer pre-screening questions given job posting, which would yield much higher coverage of screening questions for jobs, enabling relevance systems across linkedin to evaluate candidate fit to a job posting based on pre-screening qualifications data.

Because manually adding screening questions is time-consuming and is only available to jobs that are directly posted on LinkedIn, we want to design a Screening Question Generation model (SQG for short) that can automatically infer screening questions given the content of a job posting. By deploying the SQG model online, we will be able to provide screening questions to all the job postings on LinkedIn and hence greatly increases the coverage.

However, designing such a Screening Question Generation (SQG) model is not a trivial task. Although the SQG task sounds similar to the well-studied Question Generation (QG) task, none of the existing models suits our special case directly. 

Firstly, the model inputs are different. The text input of SQG task is lengthy job postings with short sentences that covers a variety of information ranging from company description, requirements, to benefits. Job postings across different industries also have vastly different language styles. On the other hand, the data of QG tasks are often shorter passages that focus on limited domains and overlaps a lot with the generated questions. As shown in Tab.~\ref{tab:qg-dataset}, the average number of words and sentences per LinkedIn job posting is larger than other common QG datasets such as SQuAD and RACE. Moreover, many QG models require additional answer text as input in order to generate questions, which is unavailable in our case.

Secondly, the objectives of SQG and QG is different. QG models are mainly designed for testing and/or improving the cognitive skills of readers, whereas in our SQG task we need to extract important qualifications and construct screening questions to best assess the qualifications of the job applicants. That being said, such objective difference prohibits us from directly applying existing QG models. In fact, directly applying QG models yield embarrassing results. Given the job posting text of Staff Software Engineer - Data Applications as input, rule-based QG methods, e.g., H\&S~\cite{heilman_question_2009} returns questions such as What is to enable others to derive near-limitless insights and intelligence from LinkedIn's data? Neural network-based QG methods, NQG for example, returns what does Experience stand for? Whereas our model returns questions such as Have you completed the following level of education: Bachelor’s Degree?

Thirdly, the mainstream QG methods, e.g., rule-based and Seq2Seq models, have their limitations thus they can not address our problems even if trained on our task-specific dataset. If we create a rule-based H\&S~\cite{heilman_question_2009} model by curating a question transducer with hand crafted patterns, it would require immense human labor and investigation. Such an approach is not scalable when we want to migrate to other languages or adding another type of question template. It will also have a sub-optimal recall due to the vastly job posting language difference between different industries. On the other hand, Seq2Seq QG models became more preferred in recent years because they are data driven hence more scalable compared to rule-based models. However, it cannot handle cases where one sentence can generate multiple questions without additional answer text as input~\cite{zhou_neural_2018,zhao_paragraph}. Also, the Seq2Seq model generates free form text questions, which is often too flexible and hence hard for job posters and even AI models to interpret, group, and categorize within a job posting or across different postings.

Lastly, majority of the QG models are designed for offline inference with a moderate latency. The inference of SQG must happen in real time right after the job description comes out. Longer online questions inference time leads to sluggish performance thus poor customer experience. There's a challenge to keep the inference latency within an acceptable range. In our work, we explored various models and listed their inference latency in Tab.~\ref{tab:qg-time}. It is clear that the latency of our current production SQG model is significantly lower than other QG models.

Recall that the screening questions used at LinkedIn is defined as (template, parameter) pairs instead of free form text to eliminate possible ambiguity. In this work, we propose a two-step SQG model named Job2Questions that given the content of a job posting, first generates all possible (template, parameter) screening question candidates, and then identifies top-k (template, parameter) screening question pairs as the output.

In candidate generation, we divide job postings into sentences and generate all question candidates by converting each sentence to (template,parameter) pairs. To get the template of the sentence, we solve multiclass classification in which one sentence is classified into one of the predefined templates. The challenge is to develop a deep, fast model that can understand the semantic meaning of the text with a small number of labeled examples. We apply deep transfer learning~\cite{chung_supervised_2018} with Deep Averaging Network to achieve both speed and accuracy. In terms of parameter entities, we developed a simple tagger based on dictionary lookup to tag out all entities out of the sentence to our best knowledge. In question ranking, we build an XGBoost pointwise ranking model to sort screening questions using extensive features from both job and question side. The details of the SQG problem definition is described in Sec.X and the proposed Job2Questions model is discussed in Sec. X.

The contributions of this work are summarized as follows:

\begin{itemize}
    \item We proposed a new Screening Question Generation (SQG) task which infers structured screening questions from job posting text to help assess job applicants. To the best of our knowledge, this is the first work on this task.
    \item We devise a general framework and data collection strategy for the SQG task.
    \item We discussed our in-production SQG solution, the Job2Questions model, and its designing details.
    \item We conducted extensive online and offline evaluation to demonstrate how SQG can help improve the hiring efficiency and user satisfaction.
\end{itemize}

\begin{table}[t]
    \caption{Statistics of popular question generation datasets.}
    \label{tab:qg-dataset}
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{l | c c}
    Dataset & Avg. words/doc & Avg. sents/doc \\
    \midrule
    SQuAD~\cite{rajpurkar_squad_2016} & $135$ & $5$ \\
    RACE~\cite{lai_race_2017} & $323$ & $18$ \\
    \midrule
    LinkedIn & $\mathbf{584}$ & $\mathbf{40}$
    \end{tabular}
    \end{adjustbox}
\end{table}

\begin{table}[t]
    \caption{Empirical CPU inference time per instance. J2Q-TC-DAN is our current in production model.}
    \label{tab:qg-time}
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c | c c | c c c}
            & Rule-based & Seq2Seq & & Our SQG Models & \\
    \midrule
    Latency & H\&S & NQG & BOW-XGBoost & \textbf{J2Q-TC-DAN} & J2Q-TC-BERT \\
    \midrule
       (ms) & $24$ms & $62$ms & $4$ms & $\mathbf{9}$ms & $100$ms 
    \end{tabular}
    \end{adjustbox}
\end{table}

\section{Related Work}

Rule-based Question Generation. Rule-based models usually transform and formulate the questions based on the text input using a series of hand-crafted rules. ELIZA [Weizenbaum, 1966] generates question responses for conversations using human-made, keyword-based rules. Mitkov, Ruslan, 2003 uses language patterns and WordNet to create multiple-choice questions. Heilman, M. and Smith, N.A., 2009 introduced a rule-based model to generate reading comprehension questions. Despite the high precision, these rule-based models are not scalable and require immense human efforts and domain-specific expertise, which is not suitable for our case where it is hard to conclude patterns for jobs from different industries.

Context-only Neural Network Question Generation. Recently, neural network models that generate questions based on the given context have shown promising results with little human intervention. Du et al., 2017and Chali et al., 2018 employed a Seq2Seq model with attention mechanism for question generation tasks and trained the model in an end-to-end fashion. None of these works are designed for generating screening questions from job posting text for applicant assessment, which is different from traditional reading comprehension question generation tasks. Moreover, the freeform questions generated by above Seq2Seq models often do not have clear-cut-intent and too flexible for job posters and downstream machine learning models to interpret and categorize. The latency of Seq2seq models is also less ideal for fast online inference.

Answer-aware Neural Network Question Generation. To simply the question generation task and handle cases where one input sentence maps to multiple questions, researchers proposed answer-aware question generation models where both the context and the answer of the target question is known. Tang et al., 2017 improved the Seq2Seq model with a global attention mechanism that leverages additional answer information in the postprocessing step by replacing out-of-vocabulary with the word in the answer having the highest relevance score among the attention distribution. Zhou et al., 2017 proposed a Seq2Seq model that takes both the context and answer as input and generates questions using answer words-copying[Gulcehre et al., 2016]. Sun, Xingwu, et al., 2018 further empower the QG model by explicitly leveraging the answer embedding and modeling the distance between the answer and the context. Gao, et al., 2019 extend the traditional QG problem to Difficulty-controllable Question Generation (DQG) in which questions were generated based on the difficulty level designated given one pair of the context and the answer.  However, the answer is not available for the screening question generation task, which means these methods are not applicable to our case. 

Applicant assessment and Person-Job fit. Our work is also closely related to person-job fit. Caldwell et al., 1990  assessed the person-job fit and competence based on interviews. Vieira et al., 2005 used skill assessment to estimate job satisfaction. Lemistre, et al., 2011 adopted an empirical mathematical model to evaluate job qualifications in terms of geographical distance and relocation. Recently, DuerQuiz has proposed to create in-depth skill assessment questions to test if the applicant is good at certain hard skills such as Machine Learning. But it does not consider other general qualifications such as education background, work authorization, year-of-experience, or soft skills. Qin et.al. proposed APJFNN which predicts person-job fit by comparing the job description and applicants’ work experience in their resume. Such a method does not have good explainability because it does not generate screening questions which can then be used to interpret why an applicant is a good or bad fit. In general, none of these person-job fit models have studied the task of modeling person-job fit by generating explicit screening questions from job postings.

\section{Problem Statement}\label{sec:problem_statement}
The Screening Question Generation (SQG for short) task aims to generate screening questions from the job posting text. Once the screening questions are generated, job applicants will provide their answers to these questions when they apply for the job. Based on the answers the applicants provide, the recruiters will identify qualified candidates based on the answers applicants provide. LinkedIn will also recommend other jobs to the applicant by matching their answers to the screening questions of other jobs and identify the ones that the applicant qualifies.

At LinkedIn, we decide to use structured screening question in the form of (template, parameter), for example, (\textsf{How many years of work experience do you have using}, \textsf{Java}), instead of freeform text for the following reasons:
\begin{itemize}
    \item \textbf{Structured questions ensure question quality}. By predefining the question types and possible parameters, we can ensure the screening question is unambiguous and reduce the chance of introducing inappropriate questions;
    \item \textbf{Structured questions has clear intent}. Unlike freeform text questions, the intent of structured questions are strictly defined by the question template. Therefore, job posters can easily group and screen candidates based on certain intent, e.g. education background, experience in multiple industries, or the list of tools they are familiar with. 
    \item \textbf{Structured questions standardize questions across jobs}. By limiting screening questions to have pre-defined templates and parameters, questions from different jobs will have exactly the same representation. This property makes it possible for us to recommend jobs that the applicants may qualify by comparing their answers to other jobs’ screening questions.
\end{itemize}

Based on the above three reasons, here we define the SQG task as inferring structured screening questions from job posting text instead of a seq2seq task which generates freeform questions from the given job posting.

\begin{figure*}[t] 
\centering
  \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=.95\textwidth]{figures/job2questions_overview.png}
  \end{subfigure}%
% \vspace{-.5cm}
  \caption{Overview of the Screening Question Generation task and its sub-tasks.}
\label{fig:sqg_overview} 
\end{figure*}

\begin{mydef}\label{def:job_sqg}
\textbf{Screening Question Generation.} Given the text of a job posting $j=\{w_1, \ldots, w_{n_w}\}$, where $w_\star$ represent words in the job and $n_w$ denotes the total number of words in the job. \textbf{Screening Question Generation (SQG)} returns $k$ top-ranked structured screening questions $\{(t, p)| t \in \mathbf{T}, p \in \mathbf{P}_t\}$, where $\mathbf{T}$ is a set of pre-defined templates, and $\mathbf{P}_t$ is a set of pre-defined parameters for template $t$.
\end{mydef}

For example, given a job posting of \textsf{Staff Software Engineer - Data Applications} posted by LinkedIn, the Screening Question Generation model should return a list of screening questions in the format of template and parameter pairs, for example, (\textsf{Have you completed the following level of education}, \textsf{Bachelor’s Degree}), and (\textsf{How many years of work experience do you have using}, \textsf{Java}).

However, designing an SQG model that can generate screening questions using the whole job posting as input is challenging. The job postings are longer and much noisy compared to the SQuAD~\cite{rajpurkar_squad_2016} dataset, where each passage is relatively short and only focuses on one topic. As we discussed previously, the average length of a job posting is four times longer than the SQuAD passages. Moreover, job postings usually cover a wide range of topics, including company description, job functions, benefits, compensation, schedules, disclaimers, and many others that are not related to the screening question generation process.

Inspired by the setting of Question Generation (QG for short) tasks, where the majority ($99.73\%$~\cite{du_learning_2017}) of the questions could be derived from a single sentence, here we hypothesize that the SQG problem can also be modeled by a sentence-level model. %To verify this hypothesis, we compute the question-to-sentence mapping and find that \hl{$X\%$} of the screening questions map to only one sentence, which supports our assumption.

Based on the above assumption, we propose a three-step sentence-level SQG framework and illustrate its overall architecture in Fig.~\ref{fig:sqg_overview}. As shown in Fig.~\ref{fig:sqg_overview}, we first tokenize the given job posting into sentences, and then we run a question template classification model to detect the most probable template for each sentence. For every sentence that has a valid, non-$\mathsf{NULL}$ template, we first use the template-dependent parameter extractor to extract possible parameters, and then construct a list of screening question candidates using the extracted parameters and the template. Lastly, we aggregate all question candidates and use a question ranking model to pick $k$ top-ranked template-parameter pairs as the final suggested screening questions for the given job posting. Next, we will provide the formal definition of the sentence-level SQG task and its sub-tasks.

\begin{mydef}\label{def:sent_sqg}
\textbf{Sentence-level Screening Question Generation}. Given job posting $j=\{s_1, \ldots, s_{n_s}\}$, \textbf{Sentence-level Screening Question Generation} extracts a list of screening question candidates $\mathbf{Q}_j = \bigcup_{s_i}^{s_i\in j}\{(t, p) | t=\textsf{TC}(s_i), p\in \textsf{PE}(s_i, t)\}$, where $\textsf{TC}$ is some question template classification model, and $\textsf{TC}$ is some parameter extraction model, and output $k$ top-ranked structured screening questions $\{(t, p)| t \in \mathbf{T}, p \in \mathbf{P}_t\}=\textsf{QR}(\mathbf{Q}_j, j, k)$, where $\textsf{QR}$ is some question ranking model.
\end{mydef}

In Def.~\ref{def:sent_sqg}, we enforce a one-to-one mapping between sentence and question template instead of sentences and questions. Based on our observation, we find that $88.9\%$ of the sentences with a non-\textsf{NULL} template only maps to one questions. The reset $11.1\%$ sentences, on the other hand, usually maps to multiple questions with the same template but different parameters. For example, \textsf{4+ years experience programming experience in Java and C/C++} can be converted into two screening questions with the same template (\textsf{How many years of work experience do you have using}, \textsf{Java}) and (\textsf{How many years of work experience do you have using}, \textsf{C/C++}).

Next, we will formally define three sub-tasks of the sentence-level SQG task, namely question template classification, template parameter extraction, and question ranking.

\begin{mydef}\label{def:tc}
\textbf{Question Template Classification}. Given a sentence $s = \{w_1, \ldots, w_{n_w}\}$ from job posting $j$ where $w$ are word tokens, \textbf{Question Template Classification} (TC) predicts the question template $t_s \in T$ of $s$ or $\textsf{NULL}$ if $s$ does not match any template.
\end{mydef}

\begin{mydef}\label{def:pe}
\textbf{Template Parameter Extraction}. Given a sentence $s = \{w_1, \ldots, w_{n_w}\}$ from job posting $j$ and predicted template $t_s$, \textbf{Template Parameter Extraction} (PE) extract a list of possible parameter values $\mathbf{P}_{s,t_s}$ from $s$ with respect to template $t_s$.
\end{mydef}

Note that for a given sentence $s$, Def.~\ref{def:tc} may return \textsf{NULL} if $s$ should not be converted into any screening question. Note that SQG is different from the traditional QG settings where the input passage always maps to one or more questions~\cite{duan_question_2017,zhao_paragraph-level_2018}. In SQG, a large portion of the sentences in the job posting is irrelevant to the qualification evaluation of an applicant, and therefore should not be converted into screening questions.

Lastly, once we get the set of screening question candidates $\mathbf{Q}_j$, we use a question ranking model to rank all the questions and return the top-k questions as the generated screening question of the job posting J.

\begin{mydef}\label{def:qr}
\textbf{Question Ranking}. Given a list of screening question candidates $\mathbf{Q}_j$, the question ranking model ranks them into an ordered question list based on $P(selected|(j,t,p))$, the probability that the job posters will add the screening question $(t,p)$ to the given job $j$.
\end{mydef}

In the next few sections, we will describe the data collection and model design for all three components of the proposed sentence-level SQG task.

\section{Data Preparation}
In this section, we will describe two methods we used, namely crowdsourcing and user feedback, to collect training and high-quality evaluation data for the template classification and question ranking tasks. Note that we leverage our existing, in-house named entity recognizer as the parameter extractor, therefore we will omit the data preparation for the entity recognizer component in this section. The statistics of the two datasets we collected in this section is described in Tab.~\ref{tab:sqg-stat}.

\begin{table}[t]
    \caption{Statistics of Screening Question Generation Dataset.}
    \label{tab:sqg-stat}
    % \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{l | r r}
    Task & Train & Test \\
    \midrule
    Question Template Classification & $7,053$ & $3,648$ \\
    Question Ranking & $88,354$ & $22,055$ \\
    \end{tabular}
    % \end{adjustbox}
\end{table}

\subsection{Question Template Classification}
Given a sentence $s$, the first step of the sentence-level SQG task is to predict its most probable question template $t$. In order to train a template classification model, we need to collect sentence-template $(s, t)$ pairs. 

\begin{table}[t]
    \caption{Examples of the crowd sourcing annotation task.}
    \label{tab:cs-example}
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabularx}{0.9\textwidth}{X}
    \toprule
    \textbf{Is the given sentence from job description directly related to the given screening question?}\\
    \midrule
    \textbf{Sentence from job description}: \\
    \quad\quad Facebook's mission is to give people the power to build community and bring the world closer together. \\
    \textbf{Screening Question}: \\
    \quad\quad How many years of work experience do you have using Facebook? \\
    \\
    \toprule
    \textbf{Is the given sentence from job description directly related to the given screening question?}\\
    \midrule
    \textbf{Sentence from job description}: \\
    \quad\quad Performing annual and periodic Fair Lending and UDAAP analysis and reporting utilizing CRA Wiz and R Studio . \\
    \textbf{Screening Question}: \\
    \quad\quad How many years of work experience do you have using R?
    \end{tabularx}
    \end{adjustbox}
\end{table}

Here we performed a crowdsourcing task to collect labeled sentence-template pairs. Tab.~\ref{tab:cs-example} shows two examples of the crowdsourcing annotation task we designed to collect labeled data. The sentences and screening questions are generated as follows. We first run entity recognizer on all sentences, and collect a list of sentences that contain valid parameters. Then for each sentence-parameter $(s, p)$ pair, we generate a screening question $(t, p)$ for $s$, where $p$ can be used as $t$'s parameter ($p \in P_t$). Lastly, we randomly sample a subset of these generated $(s, t, p)$ triples, convert them into the format shown in Tab.~\ref{tab:cs-example}, and ask human annotators to label these sentence-question pairs. We consider the sentence-template pair $(s, t)$ pair is positive if the human labeler labels at least one triple from $\{(s, (t, p))|p\in\mathbf{P}_t\}$ as directly related. Otherwise we consider that sentence $s$ maps to \textsf{NULL} template $(s, \textsf{NULL})$.

\subsection{Question Ranking}\label{sec:data_prep_qr}
As shown in Fig.~\ref{fig:sqg_overview}, once we have a list of screening question candidates, the next step is to rank them and pick the top-$k$ ranked questions as the output of the SQG model. To train such a ranking model, Because the objective of question ranking is to predict the probability of a screening question $(t,p)$ been added to job posting $j$ by the job poster, we need to collect the corresponding $(j,t,p)$ triples for model training.

Although we can ask job posters to manually add screening questions to jobs, such approach only provides positive labeled triples. The challenge for question ranking data collection is the lack of negative labeled data. The random generated negative data are easy to separate and cannot help improve the model performance. Another approach is to randomly pick job-generated screening questions that do not match job poster provided questions as negative labeled data. Such negative labeled triples may have a high false-negative rate: job posters did not add such questions because they simply forgot about it, and if we show those questions to them, they will add them to the job posting.

Therefore, to collect high-quality question ranking, we need to explicitly ask job posters to provide negative labeled data. In this work, we first designed a simplified sentence-level SQG model which is described in Sec.~\ref{sec:exp_setting} as the BOW-XGBoost model, deployed it in production to provide screening question suggestions to job posters, and then collect the labeled question ranking triples using job posters' feedbacks. Namely if a job poster accepts a suggestion or adds a new screening question, we generate a positive labeled $(j,t,p)$ triple. If job poster rejects a screening question suggestion, we generate a negative labeled $(j,t,p)$ triple accordingly. We collected $110,409$ labeled triples and group them into two triple sets $(j,t,p)\in D^+$ and $(j,t,p) \in D^-$, where $D^+$ contains all positive-labeled data and $D^-$ is a triple set of negative-labeled data.

\section{Job2Questions}\label{sec:job2questions}
After describing the problem formulation and data preparation process for each component of the sentence-level screening question generation (SQG) task, here we describe the detailed design of our production sentence-level SQG model, the Job2Questions model. We will describe its three core components as shown in Fig.~\ref{fig:sqg_overview}, namely the question template classification, question parameter extraction, and the question ranking.

\subsection{Question Template Classification}
As the first component of the Job2Questions model, question template classification takes a raw sentence as input and predicts its most probable template label, or NULL if it is not eligible. Here in this work, we treat this task as a multiclass classification task and consider template labels and the non-eligible NULL as classes. The overview of the question template classification component is shown in Fig.~\ref{fig:template_classification}. 

\begin{figure}[t] 
\centering
  \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=.95\textwidth]{figures/template_classification.png}
  \end{subfigure}%
% \vspace{-.5cm}
  \caption{Question Template Classification Model Overview.}
\label{fig:template_classification} 
\end{figure}

As shown in Fig.~\ref{fig:template_classification}, for a given sentence $s$, we first tokenize it into word or n-gram tokens $\{w_1, \ldots, w_{n_w}\}$, and then use a sentence encoder to convert the tokens into a sentence embedding vector $z_{\textsf{sent}}$. The generated sentence embedding vector $z_{\textsf{sent}}$ is then sent to a neural network model to predict its most probable class label $\hat{t}$. 

Because the training data set (around $8$k) is relatively small compared to tens of millions of jobs posted on LinkedIn, it definitely does not contain all the words in the vocabulary and does not cover all the creative ways recruiters describe job requirements. To address this issue, we decide to utilize multi-task transfer learning~\cite{pan_survey_2010} to pre-train the sentence encoding model with multiple natural language understanding tasks, and then use transfer learning to fine-tune the trained model with our question template classification task. As shown in Fig.~\ref{fig:template_classification}, we first pre-train the sentence encoder with general tasks, and then fine-tune the sentence encoder with the task-specific MLP using our template classification data. 

Here we propose two methods to encode sentence into embeddings, a simple and fast Deep Average Network (DAN)~\cite{iyyer_deep_2015} model and a more advanced Deep Bidirectional Transformers (BERT)~\cite{devlin_bert:_2018} model. We choose DAN due to its simplicity and competitive performance compared to relative computational expensive models such as CNN~\cite{jiao_convolutional_2018} and LSTM~\cite{lin_structured_2017} models. We also used BERT as our sentence encoder to see how advanced NLP model can help improve the performance in this specific task.

The DAN model first average the embedding of the input tokens into $\bar{w}$, and then pass it through two fully-connected layers to get the sentence representation $z_{sent}$.
\begin{align}
\begin{split}
    \bar{w} &= \frac{1}{n_w}\sum_i^k w_i; \\
    h_1 &= \textsf{relu}(\bar{w}W_1 + b_1); \\
    z_\textsf{sent} &= \textsf{relu}(h_1W_2 + b_2).
\end{split}
\end{align}
BERT, on the other hand, uses Transformer layer~\cite{vaswani_attention_2017} to encode the input sentence to embedding. It is defined as follows
\begin{align}
\begin{split}
    \textsf{TFLayer}(h^{n-1}) &= \textsf{FC}(\textsf{MultiAttn}(h^{n-1}));\\
    \textsf{FC}(x) &= \textsf{relu}(xW_1 + b_1)W_2 + b_2;\\
    \textsf{MultiAttn}(h^{n-1}) &= \textsf{concat}(head_1(h^{n-1}),\ldots,head_k(h^{n-1}))W^O; \\
    \textsf{head}_i(h^{n-1}) &= \textsf{softmax}\left(\frac{(h^{n-1}W_q^i)(h^{n-1}W_k^i)}{\sqrt{d_k}}\right)(h^{n-1}W_v^i).
\end{split}
\end{align}
\noindent{}where $h^{n-1}$ is the output of the previous Transformer layer. Here we use a BERT model with $8$ Transformer layers, and define the output sentence embedding $z_{\textsf{sent}}$ as the meanpooling result of the last transformer layer's output. For simplicity, we omit batch normalization~\cite{ioffe_batch_2015} and residual connections~\cite{he_deep_2016} in the equations.

After we obtain the sentence embedding $z_{\textsf{sent}}$, we then pass it through a multilayer perceptron network (MLP) where each fully-connected layer is defined as 
$$f(x) = \textsf{relu}(xW + b),$$
\noindent{}and the last layer of the MLP is defined as 
$$\hat{P} = \textsf{softmax}(f(x)W + b),$$
\noindent{}where the output $\hat{P}$ is the categorical probability distribution of each class. Finally, we pick the most probable class $\argmax(\hat{P})$ as the final predicted template label. To train the model, we use a binary-cross entropy loss 
\begin{equation}
    \mathcal{L}(P,\hat{P}) = -\sum_{i}p^i\log\hat{p}^i,
\end{equation}
\noindent{where} $P$ is the ground truth, $p^i$ and $\hat{p}^i$ are the ground truth and predicted probability of $i^{\textsf{th}}$ template respectively. We use the Adam optimizer~
\cite{kingma_adam_2017} to optimize the parameters with respect to the cross entropy loss.

\subsection{Question Parameter Extraction}

For a given job posting, we first break it down into sentences and get each sentence’s most probable template label using the above question template classification model. For all the sentences that have a valid non-NULL template that requires a template, we call the entity tagger to detect the corresponding template parameter by tagging specific type of entities from the given sentence. In our current production model, we support four types of entities, namely education degrees, tool-typed skills, spoken languages, and credentials (certifications and licenses). The challenge here is to identify entity mentions from lengthy job posting text in real time.

To tag entities from sentences, the simplest and the fastest way is to build a taxonomy where each entity has a list of surface forms, and then employ a trie-based string matching model to identify entity mentions using the developed taxonomy. 

In real-world, such a string matching approach is suboptimal because it failed to consider the context and therefore has a high false positive rate. For example, \textsf{Chinese} is mentioned in \textit{Our clients include European and Chinese companies}, but it is not a valid spoken-language mention. Another example is \textsf{bachelor} in \textit{We provide bachelor party supplies}, it does not refer to the bachelor's degree. To solve such issue, researchers have developed complicated models such as LSTM+CRF~\cite{lample_neural_2016} or LSTM+charCNN+CRF~\cite{ma_end--end_2016} to better model the mention context. However, running such a heavy model on the full job posting text is time consuming and may significantly increase our service latency. 

As an alternative approach, we first tag entities using the above trie-based string match method, and then score each entity mention using a logistic regression model with contextual features such as POS tag, mention frequency, context n-grams, and the cosine similarity between the FastText~\cite{joulin_bag_2016} embeddings of the mention and its context. Finally, entity mentions with a confidence score that passes the given threshold will be considered as template parameters of the given sentence $s$ and template $t$.  


\subsection{Question Ranking}\label{sec:job2questions_question_ranking}
After we get all the question candidates in the format of template label and parameter pairs $(t,p)$ from the given job posting, the next step is to rank the candidates and find questions that are helpful for the hiring process. Because determining whether or not a screening question is helpful for the hiring process is non-trivial, in this work we assume recruiters and job posters know what screening questions are best for the hiring process. Hence, we use the screening questions added and rejected by them as the ground truth labels and define the question ranking objective as predicting the likeliness of a job poster adds a screening question candidate $(t,p)$ to a job posting $j$. 
\begin{equation}\label{eq:qr_prob}
    	\textsf{Pr}(\textsf{accepted} | j, t, p) = sigmoid(f(x_{j,t,p})),
\end{equation}
\noindent{where $f$ is the scoring function, $x_{j, t, p}$ is the feature vector with respect to the given job $j$, template label $t$, and parameter $p$ triple.}

The features we used to construct $x_{j,t,p}$ can be group into three groups, job-side features, question-side features and job-question interactive features. 

\textbf{Job-side features}: the feature is purely extracted and associated with the job posting itself. The whole set of job-side feature is listed in Tab.~\ref{tab:QR_job_side_features}

\begin{table}[ht]
    \caption{Question ranking job-side features.}
    \label{tab:QR_job_side_features}
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{l | c }
        Feature & Description\\
        \midrule
        company size & the population size of the company who posted the job \\
        industries & the industries that the job position belongs to\\
        industry category & the industry category that the job position belongs to\\
        location & the location of the job\\
        experience level & the experience level that the job requires\\
        years of experience & the least years of working experience that the job requires\\
        roles & the role of the position that the job offers\\
        occupations & the job occupations\\
        specialties & the specialties the job requires\\
        parent specialties & the specialties in more general scope\\
        employment status & the employment status of the job\\
        functions & the job functions\\
        seniority & the seniority the job requires\\
        title & job titles\\
        super title & the job titles in more general scope
        \end{tabular}
    \end{adjustbox}
\end{table}

\textbf{Question-side features}: the features extracted purely from the generated questions. The whole feature list is shown in Tab.~\ref{tab:QR_question_side_features}

\begin{table}[ht]
    \caption{Question ranking question-side features.}
    \label{tab:QR_question_side_features}
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{l | c }
        Feature & Description\\
        \midrule
        template type & the template type that the question belongs to\\
        parameter value & the parameter value of the question\\
        template confidence score & the confidence score for the question belonging to one of the template types\\
        question ranking position & the ranking position of the template with the highest confidence score among all template types\\
        job skill score & the confidence score of the skills the questions ask \\
        \end{tabular}
    \end{adjustbox}
\end{table}

\textbf{Job-Question interactive features}: We use the pointwise mutual information (PMI) score between the job-side features and the job-side features as our interaction feature. The PMI is defined as follows:
\begin{equation}\label{eq:qr_interaction_feature_pmi}
    	\textsf{PMI}(j ; q) = log\frac{\textsf{Pr}(j,q)}{\textsf{Pr}(j)\textsf{Pr}(q)},
\end{equation}
where $j$ is the job-side feature and $q$ is the question-side feature. The PMI value quantifies the discrepancy between the probability of correspondence of a job-side and a question-side event given both joint and individual distribution. Tab.~\ref{tab:QR_num_interactive_features} shows the number of features we picked from job and question sides to generate interactive features. And Tab.~\ref{tab:QR_interactive_features} demonstrate samples of interaction features.
\begin{table}[ht]
    \caption{Job-Question number of interactive features (PMI features).}
    \label{tab:QR_num_interactive_features}
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{l | c | c | c}
        & Question-side & Job-side & Interactive \\
        \midrule
        feature number & 5 & 27 & 135 (5x27) \\
        \end{tabular}
    \end{adjustbox}
\end{table}

\begin{table}[ht]
    \caption{Job-Question interactive features (PMI features).}
    \label{tab:QR_interactive_features}
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{l | l }
        Question-side feature & Job-side feature\\
        \midrule
        template \#1 & company size \\
        template \#2 & company size\\
        parameter value of template \#1 & industries\\
        parameter value of template \#2 & location\\
        \end{tabular}
    \end{adjustbox}
\end{table}

After describing the feature vector $x_{j,t,p}$, next we present the scoring function $f$. Here we use XGBoost as the scoring function and therefore rewrite Eq.~\ref{eq:qr_prob} as 

\begin{equation}
    \textsf{Pr}(\textsf{accepted} | j, t, p) = sigmoid\left(\sum_k f_k(x_{j,t,p})\right)
\end{equation}
\noindent{}where $f_k$ is the $k^\textsf{th}$ tree of the model. We use the following loss function to optimize the question ranking model
\begin{equation}
\begin{split}
    \mathcal{L} =& -\sum_{\langle j,t,p\rangle\in\mathbf{D}^+}\log\left(\sum_{k}f_k\left(x_{j,t,p}\right)\right) \\
    &- \sum_{\langle j,t,p\rangle\in\mathbf{D}^-}\log\left(1 - \sum_{k}f_k\left(x_{j,t,p}\right)\right) + \sum_{k}\Omega(f_k),
\end{split}
\end{equation}
\noindent{}where $D^+$ and $D^-$ are the positive and negative $(j, t, p)$ triple sets collected using the job posters’ feedback described in Sec.~\ref{sec:data_prep_qr}. $f_k$ represents the $k^\mathsf{th}$ tree in the boosted-tree model, $\Omega(f_k) = \gamma T + \frac{1}{2}\lambda||\mathbf{w}||^2$ is the regularization term that penalizes the complexity of tree $f_k$, in which $T$ denotes the number of leaves in tree $f_k$, $\mathbf{w}$ is the leaf weights, $\gamma$ and $\lambda$ are the regularization parameters.


\section{Experiments}
In this section, we conducted extensive evaluations on the proposed Job2Questions (J2Q for short) model. The promising offline and online A/B test results demonstrate the effectiveness of the proposed Job2Questions model in terms of providing high quality screening question suggestions. 

\subsection{Experiment Setting}\label{sec:exp_setting}

In this section, we evaluated the following variants of the question template classification model:
\begin{itemize}
    \item \textbf{BOW-XGBoost}: this is a non-neural network baseline model which tokenize the input sentence into bag-of-word vectors and then trained an XGBoost~\cite{chen_xgboost_2016} model to predict the template label.
    \item \textbf{J2Q-TC-NNLM}: the J2Q template classification model variant which uses a simple feed-forward neural network language model (NNLM)~\cite{bengio_neural_2003} as the sentence encoder.
    \item \textbf{J2Q-TC-DAN}: the J2Q template classification model with deep averaging networks~\cite{iyyer_deep_2015} as the sentence encoder.
    \item \textbf{J2Q-TC-CNN}: the J2Q template classification model with CNN-based universal sentence encoder~\cite{jiao_convolutional_2018} as the sentence encoder.
    \item \textbf{J2Q-TC-BERT}: the J2Q template classification model with BERT~\cite{devlin_bert:_2018} as the sentence encoder.
\end{itemize}
All above models are trained using the same dataset as described in Tab. X. For neural network J2Q-TC-$\star$ models, we use the public-available pre-trained models~\cite{cer_universal_2018,devlin_bert:_2018} as initialization and fine-tune them accordingly. For J2Q-TC-\{NNLM, DAN, CNN\}, we set the learning rate to $1e-3$, batch size to $256$, and drop-out rate to $0.4$. For BERT, we further truncate/pad the input sentence to $32$ tokens and set the learning rate to 5e-5. All models are trained for at most $100$ epochs with a $3$-layer MLP.

As for the question ranking model, here we evaluate the following variants:
\begin{itemize}
    \item \textbf{Rule-based}: It is a non-machine learning and we use it as our baseline. It sorts questions based on the confidence score outputted by the template classification model and then re-rank them using the business rules, e.g. education and work authorization questions always rank at the top.
    \item \textbf{J2Q-QR-logistic-regression}: The logistic regression model that ranks candidates via binary classification. 
    \item \textbf{J2Q-QR-XG-Boost-pointwise}: The proposed question ranking model trained with a pointwise loss.
    \item \textbf{J2Q-QR-XG-Boost-pairwise}: The proposed question ranking model trained with a pairwise loss.
\end{itemize}
The J2Q question ranking model is trained with tracking data collected via job posters feedback. Total 110,409 labeled $(j, t, p)$ labeled triples were collected as our question ranking dataset in which 70\% of the them is used for training, 20\% of them is used for evaluation and 10\% of the data is used for validation. We explored and anchored the hyper-parameter in tree-based models (i.e. J2Q-QR-XG-Boost-pointwise and J2Q-QR-XG-Boost-pairwise models). Specifically, in both XG-Boost models, 100 trees with 5 for the maximum depth of each one were used; gbtree was employed as the booster; eta is set to 0.7 and gamma is fixed to 0. As for evaluation metrics, we optimized receiver oper-ating characteristic curve (AUROC) and normalized discounted cumulative gain (NDCG) for the pointwise and pairwise XG-Boost model respectively. Additionally, we partitioned the data and trained the XG-Boost models on Hadoop clusters. We set the number of executors in clusters to 50 so that the distributed shuffle of data will succeed while each output partition will contain just a small amount of data (i.e. 2208 sentences for each executor in our case).


\subsection{Offline Evaluation}

\begin{table*}[ht]
    \caption{Offline Evaluation of Question Template Classification.}
    \label{tab:tc-eval}
    \centering
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{l|c|cccccccccccccc}
         &  & \multicolumn{2}{c}{NULL} & \multicolumn{2}{c}{Work Auth} & \multicolumn{2}{c}{Sponsorship} & \multicolumn{2}{c}{Education} & \multicolumn{2}{c}{Language} & \multicolumn{2}{c}{Credential} & \multicolumn{2}{c}{Tools} \\
        Model & Overall Acc. & Prec. & Rec. & Prec. & Rec. & Prec. & Rec. & Prec. & Rec. & Prec. & Rec. & Prec. & Rec. & Prec. & Rec. \\
        \midrule
        BOW-XGBoost & $0.3547$ & $0.1336$ & $\mathbf{0.5988}$ & $0.4118$ & $0.1386$ & $0.5000$ & $0.0051$ & $0.5644$ & $0.8519$ & $\mathbf{0.9888}$ & $0.3346$ & - & - & $0.5329$ & $0.4863$ \\
        J2Q-TC-CNN & $0.8640$ & $0.5408$ & $0.2536$ & $0.9397$ & $0.9639$ & $0.9488$ & $0.9915$ & $0.9199$ & $0.8857$ & $0.9328$ & $0.9680$ & $0.6865$ & $\mathbf{0.9227}$ & $0.9037$ & $0.8151$ \\
        J2Q-TC-NNLM & $0.8765$ & $0.6250$ & $0.2871$ & $0.9425$ & $0.9716$ & $0.9514$ & $0.9915$ & $0.8984$ & $0.9343$ & $0.9598$ & $0.9710$ & $0.7019$ & $0.9040$ & $0.9193$ & $0.8374$ \\
        J2Q-TC-DAN & $0.8798$ & $0.6330$ & $0.3301$ & $0.9333$ & $\mathbf{0.9742}$ & $0.9538$ & $0.9887$ & $0.9056$ & $0.9314$ & $0.9648$ & $0.9564$ & $0.7227$ & $0.8827$ & $0.9068$ & $0.8664$ \\
        J2Q-TC-BERT & $\mathbf{0.9138}$ & $\mathbf{0.6688}$ & $0.4928$ & $\mathbf{0.9592}$ & $0.9691$ & $\mathbf{0.9592}$ & $\mathbf{0.9944}$ & $\mathbf{0.9282}$ & $\mathbf{0.9600}$ & $0.9655$ & $\mathbf{0.9767}$ & $\mathbf{0.8564}$ & $0.8747$ & $\mathbf{0.9197}$ & $\mathbf{0.9465}$
        \end{tabular}
    \end{adjustbox}
\end{table*}

\begin{figure*}[ht] 
\centering
  \begin{subfigure}[b]{0.25\linewidth}
    \centering
    \includegraphics[width=.9\textwidth]{figures/parameters/learning_rate.png}
  \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
    \centering
    \includegraphics[width=.9\textwidth]{figures/parameters/dropout_rate.png}
  \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
    \centering
    \includegraphics[width=.9\textwidth]{figures/parameters/batch_size.png}
  \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
    \centering
    \includegraphics[width=.9\textwidth]{figures/parameters/mlp_layers.png}
  \end{subfigure}%
% \vspace{-.5cm}
  \caption{Hyper-parameter sensitivity test for the in production J2Q-TC-DAN model.}
\label{fig:hyper_parameter_test} 
\end{figure*}

\begin{table*}[ht]
    \caption{Offline Evaluation of Question Ranking Model.}
    \label{tab:qr_offline_eval}
    \centering
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{l|l|l|l|l}
                          & Rule-based & J2Q-QR-logistic-regression & J2Q-QR-XG-Boost-pointwise & J2Q-QR-XG-Boost-pairwise \\ \hline
            Overall AUROC & 64.08\%    & 80.14\%                    & 82.79\%                   & 81.75\%                  \\
            Overall AUPRC & 61.73\%    & 75.07\%                    & 79.55\%                   & 78.06\%                 
        \end{tabular}
    \end{adjustbox}
    
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{c|ccc|ccc|ccc|ccc}
             & \multicolumn{3}{c|}{Rule-based} & \multicolumn{3}{c|}{J2Q-QR-logistic-regression} & \multicolumn{3}{c|}{J2Q-QR-XG-Boost-pointwise} & \multicolumn{3}{c}{J2Q-QR-XG-Boost-pairwise} \\
             & Precision    & Recall     & NDCG      & Precision     & Recall      & NDCG       & Precision     & Recall      & NDCG       & Precision     & Recall      & NDCG      \\ \hline
            @1   & 68.76\%      & 55.73\%    & 0.6876    & 82.24\%       & 67.39\%     & 0.8224     & 83.26\%       & 68.17\%     & 0.8326     & 83.91\%       & 68.70\%     & 0.8391    \\
            @3   & 45.12\%      & 89.85\%    & 0.8117    & 48.65\%       & 96.30\%     & 0.9086     & 48.62\%       & 96.20\%     & 0.9117     & 48.91\%       & 96.68\%     & 0.9175    \\
            @5   & 44.23\%      & 99.10\%    & 0.8546    & 44.50\%       & 99.57\%     & 0.9227     & 44.46\%       & 99.52\%     & 0.9259     & 44.51\%       & 99.58\%     & 0.9297    \\
            @all & 44.23\%      & 100\%      & 0.8586    & 44.23\%       & 100\%       & 0.9246     & 44.23\%       & 100\%       & 0.9280     & 44.23\%       & 100\%       & 0.9315   
        \end{tabular}
    \end{adjustbox}
\end{table*}

\begin{table*}[ht]
    \caption{Question ranking feature ablation study.}
    \label{tab:qr_feature_ablation_study}
    \begin{tabular}{l|cccccccc}
        \multicolumn{1}{c|}{\multirow{2}{*}{}} & \multirow{2}{*}{Overall AUROC} & \multirow{2}{*}{Overall AUPRC} & \multicolumn{2}{c}{Precision} & \multicolumn{2}{c}{Recall} & \multicolumn{2}{c}{NDCG} \\
        \multicolumn{1}{c|}{}                  &                                &                                & @1            & @3            & @1           & @3          & @1          & @3         \\ \hline
        without job-side feature               & 81.66\%                        & 77.72\%                        & 84.32\%       & 48.88\%       & 69.07\%      & 96.62\%     & 0.8432      & 0.9188     \\
        without question-side feature          & 80.41\%                        & 76.05\%                        & 82.57\%       & 48.62\%       & 67.76\%      & 96.24\%     & 0.8257      & 0.9097     \\
        without interaction feature            & 81.52\%                        & 78.11\%                        & 84.16\%       & 48.81\%       & 69.00\%      & 96.50\%     & 0.8416      & 0.9173     \\
        all feature                            & 81.75\%                        & 78.06\%                        & 83.91\%       & 48.91\%       & 68.70\%      & 96.68\%     & 0.8391      & 0.9175    
    \end{tabular}
\end{table*}

\subsubsection{Question Template Prediction.} We evaluate the question template classification performance on the crowdsourcing question template classification dataset described in Tab.~\ref{tab:sqg-stat}, which contains $6$ different template labels and a special label NULL for sentences that cannot be convert into questions. We report the precision/recall of each template label and the overall accuracy in Tab.~\ref{fig:template_classification}. We found that all deep learning models outperformed the BOW baseline by a large margin, and BERT yields the best overall accuracy, outperforming the second best DAN model by $3.9\%$. However, as shown in Tab.~\ref{tab:qg-time}, the CPU inference time of BERT ($100$ms) is $10$-times longer than the DAN model ($9$ms), making it less practical for online inference when running on CPUs. 

%Because we want to perform template classification in real time, we also measured the model inference latency on CPUs and summarized it in Tab. X. We can see that although using BERT as the sentence encoder improves the overall accuracy by 3.5\% compared to simpler sentence encoders such as DAN, the inference latency is almost 10 times longer than the DAN model, which makes it impractical for online inference. In fact, if we treat the BOW-XGBoost model as the baseline and compute the accuracy improvement per millisecond for each model, we can see J2Q-TC-DAN is actually the most “cost-effective” one which improves the overall accuracy by X\% with a latency of Y ms.

\subsubsection{Hyper-parameter Test.} To understand how different hyper-parameters affect the model's performance, we tested different configurations on the learning rate, dropout rate, batch size, and the number of MLP layers. As shown in Fig.~\ref{fig:hyper_parameter_test}, the performance of the J2Q-TC-DAN model is mostly insensitive to its hyper-parameters besides the dropout rate, which is expected. Using a larger batch size slightly hurts the performance of our model due to overfitting~\cite{keskar_large-batch_2017}. Lastly, we found that using three-layer MLP works the best for our question template classification task.

\subsubsection{Question Ranking.} To evaluate the performance of the question ranking model, here we use $22,055$ (job, template, parameter) triples from $6,675$ jobs as the evaluation data. We evaluate the ranking models using following metrics: 
\begin{itemize} 
    \item \textbf{Overall metrics}: the overall area under the receiver operating characteristic curve (AUROC); the overall area under the precision-recall curve (AUPRC).
    \item \textbf{Per-job level metrics}: precision at k (precision@k); recall at k (recall@k); and normalized discounted cumulative gain at k (NDCG@k). 
\end{itemize}
Using metrics above, we evaluated all 4 question ranking models defined in Sec.~\ref{sec:exp_setting}. Tab.~\ref{tab:qr_offline_eval} shows the performance specifics for the models. Generally speaking, the rule-based model got beaten by the machine learning models in terms of all evaluation metrics. The logistic regression model did a decent job but is still not as good as tree-based XG-Boost models. J2Q-QR-XG-Boost-pointwise model performs the best in terms of overall AUROC and AUPRC while J2Q-QR-XG-Boost-pairwise model outperforms other three models in terms of per-job level metrics, i.e. precision at k, recall at k and NDCG at k. It makes perfect sense for the tree-based models since J2Q-QR-XG-Boost-pointwise optimized the overall AUROC directly and J2Q-QR-XG-Boost-pairwise took NDCG as its objective function to maximize. In practical terms, we chose J2Q-QR-XG-Boost-pairwise as our online solution for question ranking since we rank questions in job-level thus the ranking results in per-job level make more sense in our case. 

\subsubsection{Feature Ablation Study.} 
We executed a feature ablation study using the J2Q-QR-XG-Boost-pairwise model. Namely we splitted and categorized the feature set into job-side features, question-side features and interactive features defined in ~\ref{sec:job2questions_question_ranking}. By removing one source of features from all features at each time and conducted individual experiments for each variants to filter out and remain the most important features. Tab.~\ref{tab:qr_feature_ablation_study} shows the result of the ablation study. We care about the per-job level metrics the most because we ranking questions within a job posting. (TODO: do we need to remove the overall metrics in ablation study?) The results suggest that all sources of features (i.e. job-side, question-side and interactive features) positively contributed to the model and should be retained to be used by the model since the performance dropped when removing either one source from all. Specifically, we can conclude that the question-side features played the most important part in the ranking job because the performance of all metrics dropped most significantly when removing question-side features, followed by the job-side features and the interactive features. Besides, given there’s only slightly performance improvement by adding the interaction features, we gained the insight that the correlation between job-side and question-side features can mostly be captured by our J2Q-QR-XG-Boost-pairwise model without manually adding additional insight.

\subsubsection{Feature Importance.} 
We visualize the importance of features using the importance score in XG-Boost models. Tab.~\ref{tab:qr_feature_importance} lists out top 3 features among all features (job-side, question-side and interactive) among all features ranked by the importance score (i.e. the importance score sums to 1 for all features) in descending order. As is shown in Tab.~\ref{tab:qr_feature_importance}, the most important feature is pmi which is from interactive features followed by the template classification confidence score and job functions that from question-side and job-side features respectively.


\begin{table}[H]
    \caption{Question ranking feature importance.}
    \label{tab:qr_feature_importance}
    \begin{tabular}{l|c}
        \textbf{Feature}    & \multicolumn{1}{l}{\textbf{Importance score}} \\ \hline
        pmi                 & 0.6111313203                                  \\
        TC confidence score & 0.1345943981                                  \\
        job functions       & 0.03164787206                                
    \end{tabular}
\end{table}


\subsection{Online Evaluation}
\subsubsection{Screening Question Suggestion.} As mentioned previously, when posting jobs on LinkedIn, the posters will be able to manually add screening questions. Here we deployed the BOW-XGBoost and DAN-based Job2Questions model online to provide screening question suggestions to the job posters. We ramped two models to $50\%$ of LinkedIn's traffic for two weeks and compared them against a baseline model, which simply extracts parameters from job posting and create questions accordingly. The metrics we tracked are as follows:

\begin{itemize}
    \item \textbf{Acceptance Rate}: the ratio between accepted and all suggested screening questions,
    \item \textbf{Suggestion Rate}: the ratio between jobs that receive suggestions and all jobs posted on LinkedIn.
    \item \textbf{Adoption Rate}: the ratio between jobs with screening questions and all jobs posted on LinkedIn.
\end{itemize}

As shown in Tab.~\ref{tab:ab_question_suggestions}, the proposed Job2Questions model significantly improves both the model precision and coverage. We believe the accuracy improvement is due to the expressive power of neural network models. The increase in coverage, on the other hand, is because the deep transfer learning gives good generalization ability to our model.

\begin{table}[H]
    \caption{Online A/B test of Screening Question Suggestions.}
    \label{tab:ab_question_suggestions}
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{l | c c c}
        Model & Acceptance Rate & Suggestion Rate & Adoption Rate\\
        \midrule
        BOW-XGBoost & $+31.06\%$ & $+40.86\%$ & $+14.26\%$\\
        Job2Questions & $+\mathbf{53.10}\%$ & $+\mathbf{59.92}\%$ & $+\mathbf{22.17\%}$ \\
        \end{tabular}
    \end{adjustbox}
\end{table}

\begin{figure}[ht] 
\centering
  \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=.95\textwidth]{figures/good_fit.png}
  \end{subfigure}%
% \vspace{-.5cm}
  \caption{Applicant's good fit rating versus number of screening questions they answered correctly.}
\label{fig:good_fit_rating} 
\end{figure}

\subsubsection{Job Applicant Quality.} After the proposed Job2Questions model is deployed, we also analyzed how providing screening questions can help improve the hiring efficiency in terms of job applicant quality. 
We first look at how screening questions help identify qualified applicants in around $20$M job applications. As shown in Fig.~\ref{fig:good_fit_rating}, we found that if the applicant does not answer any screening questions correctly, only $18.67\%$ of the applications are rated as a good fit by the recruiter. But if the applicant answered at least one screening question correctly, the good fit rating increases to $23\%$ ($+23.19\%$).

Because recruiters often receive a large amount of applicants per job, it is impractical for them to review all applications. Therefore they tend to sort the applicants first and only review the top-ranked candidates. Here at LinkedIn we sort the candidates using some relevance model to predict if an applicant is a good fit. As an alternative, we developed another ranking model that simply sort applicants based on the favorable of their answers to the screening questions. 
We conducted a $50$-$50$ A/B test for one month and measured the good/bad fit rating the recruiters gave to the candidates they have contacted. We found that ranking applicants by screening question answers can improve the applicant good fit rate by $7.45\%$ and reduce the bad fit rate by $1.67\%$. This means the screening questions can help the recruiters surface qualified applicants and therefore improve the hiring efficiency.

\subsubsection{Screening Question-based Job Recommendation.} We also conducted another applicant-side analysis to see if screening questions can help them apply to jobs they qualify. To be specific, we applied our Job2Questions model to all jobs available on LinkedIn, and then trained a new job recommendation model (JYMBII) using screening questions and applicant answers as additional features. We observed that when LinkedIn members applying for jobs suggested in the job recommendation email, they are $46\%$ more likely to get a good fit rating if the job is suggested by the JYMBII + screening question model.

\section{Conclusions and Future Work}
In this work, we proposed a novel Screening Question Generation (SQG) task, which generates screening questions based on the job posting text. We also proposed a general candidate-generation-and-ranking SQG framework to solve this problem. We presented the details of LinkedIn's production SQG solution, the Job2Questions model, including the data preparation, deep transfer learning-based question template classification modeling, parameter extraction, and XGBoost-based question ranking. The extensive online and offline evaluations demonstrate the effectiveness of the Job2Questions model. As for future work, we plan to investigate into more advanced question ranking methods and extending the model to support multiple languages.
